Chasing Carbon: The Elusive Environmental Footprint of Computing

Given recent algorithm, software, and hardware innovation, computing has enabled a plethora of new applications. As computing becomes increasingly ubiquitous, however, so does its environmental impact. This paper brings the issue to the attention of computer-systems researchers. Our analysis, built on industry-reported characterization, quantifies the environmental effects of computing in terms of carbon emissions. Broadly, carbon emissions have two sources: operational energy consumption, and hardware manufacturing and infrastructure. Although carbon emissions from the former are decreasing thanks to algorithmic, software, and hardware innovations that boost performance and power efficiency, the overall carbon footprint of computer systems continues to grow. This work quantifies the carbon output of computer systems to show that most emissions related to modern mobile and data-center equipment come from hardware manufacturing and infrastructure. We therefore outline future directions for minimizing the environmental impact of computing systems.

==> text/analytical.tex <==
\section{Modeling hardware carbon footprint}

To optimize the environmental impact of computing systems, the first step is to provide tools and methodologies to characterize the design space of systems across the computing stack. 
Following the analysis thus far, proposed methodologies must unify both design time decisions and run-time workload characteristics.
Finally, given emerging workloads (e.g., AI, robotics, AR/VR, autonomous driving) will run across a collection of mobile and datacenter scale systems, methodologies for quantifying carbon emissions must extrapolate to both scenarios.
In this section, we propose a first-order analytical model to quantify the carbon emissions from both operational, energy consumption and hardware manufacturing.
While power and energy modeling has been extensively studied in the systems and computer architecture community, we augment the models to incorporate emerging renewable energy technology. 
To model hardware manufacturing overheads, we provide first order carbon footprint models for compute, memory, and storage components in modern systems. 
We hope the proposed model provides a foundation for future work to build ontop of for more sophisticated methodologies, validate across a wider array of platforms, and optimize environmental footprints of mobile and datacenter scale hardware.

\subsection{Analytical model}
As previously mentioned, it is important to consider the carbon footprint of both operational, energy consumption as well as hardware manufacturing.
Thus, to enable directly comparing carbon emissions from operational, energy consumption and hardware manufacturing Equation~\ref{eqn:cf} independently combines both components for modeling carbon footprint.

\begin{equation}
CF = OP_{CF} + HW_{CF}
\label{eqn:cf}
\end{equation}

\subsection{Modeling carbon emissions from energy consumption}
Here we dissect the carbon footprint from operational, energy consumption.
First, we evaluate the average power consumption of a workload running on a given hardware platform, as shown in Equation~\ref{eqn:power}. 
$UE$ represents utilization effectiveness and overheads in power delivery; $TDP$ represents hardware thermal design power; $Util$ represents average utilization of the hardware resource.
For datacenter, $UE$ follows efficiency metrics such as \textit{PUE}, typically between 1.1 and 1.5 for modern warehouse scale datacenter~\cite{}; for mobile devices, $UE$ translates to battery charging efficiency, typically between \fixme{1.1} and 1.2 for modern mobile phones~\cite{apple phones}.
While the model focuses on compute (SOC), memory, and storage resources it can be extended to consider additional components. 
Furthermore, while here we consider an analytical model, power consumption can also be evaluated with higher fidelity methodologies based on detailed performance counters and empirical measurements~\cite{}. 

\begin{align}
Power &= UE \times \left( \sum_{r}^{soc,memory,storage} TDP_{r} Util_{r} \right) ~\label{eqn:power}\\
OP_{CF} &= EnGen \times \left(T \times Power\right) ~\label{eqn:opcf}
\end{align} 

Equation~\ref{eqn:opcf} translates the power consumption to overall carbon footprint.
Here $T$ represents the time span for running the particular workload and hardware platform.
$EnGen$ represents the efficiency of generating renewable energy in terms of grams of \co~emitted per kWh.
Table~\ref{tab:energy} shows $EnGen$ for a range of ``brown'' and ``green'' energy sources. 
Recall that $EnGen$ is especially important to consider for datacenter scale execution and varies not only based on energy source but also on geographic location.


%Operational footprint is based on the utilization of each hardware resource, $r$, and its TDP~\cite{}.
%UE computes the wasted power from driving the hardware substrate.
%In the context of datacenters, UE refers to PUE --- roughly 1.1 for warehouse scale datacenters (Google/Facebook)~\cite{}.
%T is Time.
%EnGen is the efficiency of generating energy based on the energy source such as coal, gas, bio-mass, solar, geothermal, hydropower, nuclear, and wind.

\subsection{Modeling carbon emissions from hardware manufacturing}
In addition to operational energy consumption, here we disssect the carbon footprint from hardware manufacturing.

\begin{equation}
HW_{CF} =  \sum_{r}^{soc,memory,storage} HW_{r}~\label{eqn:hw}
\end{equation} 

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{plots/memory_storage_cf_pareto.pdf}
  \vspace{-1em}
  \caption{Pareto frontier between DRAM, NAND Flash, and SSD storage capacity and carbon footprint. 
  Higher capacity NAND Flash memories offer higher carbon footprint per stroage efficiencies as compared to DRAM memories.}
  \label{fig:memory_storage_cf_pareto}

\end{figure}

\textbf{Memory and storage footprints.} Emissions hardware manufacturing are based on the aggregate footprint of each hardware resource, $r$, including SoC, memory, and storage.
Figure~\ref{fig:memory_storage_cf_pareto} illustrates the Pareto-frontier between carbon footprint efficiency in terms of grams of \co~per gigabyte of storage and memory storage capacity.
The data is based on the manufacturing carbon footprint for DRAM and NAND Flash systems from SK Hynix~\cite{}.
As expected, DRAM memories have lower storage capacity than NAND Flash systems.
Similar to storage density, where DRAM has lower density than NAND Flash, DRAM memories have higher carbon footprints per gigabyte than NAND Flash.
For instance, 50nm DDR3 has a carbon footprint of 600 g \co~per GB while 30nm NAND Flash has a carbon footprint of 31 g \co~per GB, almost 20$\times$ lower.
In addition to hardware manufacturing measurements from SK Hynix, across Apple's mobile devices (e.g., phones, tablets, laptops, wearables), we find that the carbon footprint of storage is 8.6 gram \co~per GB with a standard deviation of 1.7 gram \co~per GB. 
The absolute carbon footprints are shown in Table~\ref{tab:hw_carbon} and can be used to model hardware manufacturing overheads in Equation~\ref{eqn:hw}. 


\textbf{SoC footprint.} In addition to the carbon footprint of memory and storage, Table~\ref{tab:hw_carbon} also estimates the carbon footprint of SoC hardware. 
We estimate carbon footprint of SoC hardware based on interpolating SoC carbon footprints across Apple's mobile devices.
First, we assume \fixme{33}\% of Apple's carbon footprint comes from integrated circuits --- SoC, memory, and storage.
Next, we estimate SoC hardware footprints by subtracting out memory and storage footprints, based on Table~\ref{tab:hw_carbon}, from Apple's 2019 iPhones (i.e., iPhone 11, 11 Pro, 11 Pro Max, X, and SE).
Considering the die area of different SoC's used in the platforms we find the carbon footprint to be 273 $\pm$ 46 gram \co~per mm$^2$. 

\textbf{Modeling mobile phone footprints.} Table~\ref{tab:pixel_hw_estimate} illustrates the fidelity of proposed model on predicting hardware manufacturing overheads.
We assume Google Pixel devices have similar integrated circuit footprint (i.e., \fixme{33\%}) compared to Apple's mobile devices.
Based on the assumption, the model has a 9.2\% error on average.
The results demonstrate the first-order model can be used for future system and hardware design optimization. 

% Something about needing more data on individual resources - like Intel CPUs, networking, etc. to get more accurate breakdowns for not only mobile but also datacenter hardware. 



\input{text/table_hw_CF}

\input{text/pixel_hw_estimate}


==> text/motivation.tex <==
\section{Hardware life cycle}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{figures/HW_life_cycle.pdf}
  \vspace{-5em}
  \caption{ End to end hardware cycle includes hardware manufacturing, transport, use, and recycling.
  Operational carbon emissions (Opex-related carbon footprint) is based on \textit{use}; Capex carbon emissions result from aggregating manufacturing, transport, and recycling.}
  \label{fig:life_cycle}

\end{figure}

Figure~\ref{fig:life_cycle} illustrates the end to end hardware life cycle consisting of manufacturing, product transport, product use, and recycling.
The phases come from environmental life cycle analysis, applied to various products beyond computing technology, that aims to quantify the overall emissions for individual items~\cite{}.
Below we describe the hardware life cycle in the context of systems and computer architecture:


\begin{itemize}

\item \textbf{Production} Carbon footprint from procuring raw materials, manufacturing hardware, fabrication labs, assembly, and packaging. 

\item \textbf{Transport} Carbon footprint from transporting produced hardware to the point of use including customers and warehouse-scale datacenters.

\item \textbf{Use} Carbon footprint from the operational use of the hardware including static and dynamic power consumption, PUE-overheads in the datacenter, and battery-efficiency overheads in mobile platforms.

\item \textbf{Recycling} Carbon footprint from recycling hardware systems. A subset of recycled materials, such as cobalt in mobile devices, are used in building future systems.
\end{itemize}

In this work, we show that it is important to consider carbon emissions from each life cycle phase --- not only use --- when optimizing computer systems' environmental footprint.
Analagous to capex versus opex components in building datacenters, researchers and system designers must consider capital and operational carbon emissions.

\subsection{Capital versus operational emissions}
Systems and hardware are typically optimized for run-time characteristics such as performance, performance per Watt, or energy~\cite{}. 
The run-time metrics allow system designers and researchers to not only improve performance and application-level quality of service, but also indirectly reduce carbon footprint by optimizing energy consumption.
To directly optimize carbon footprint of hardware platforms researchers must consider the end to end hardware life cycle including manufacturing, product transport, product use, and recycling~\cite{apple, microsoft, google}. 
Similar to capex versus opex overheads in warehouse-scale datacenters, opex-related carbon emissions come from product use; capex-related emissions come from hardware manufacturing, product transport, and recycling.

For the purposes of this study, we focus our discussion on the two salient phases of the hardware life cycle --- manufacturing and product use. 
Based on the characterization shown in this paper, the majority of carbon emissions for both datacenter- and mobile-scale systems arise from manufacturing and product use.
Transport and recycling, while important aspects to consider overall, comprise a small fraction of overall carbon emissions.

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{plots/apple_breakdown.pdf}
  \vspace{-1em}
  \caption{ Apple's company level carbon emission breakdown. Manufacturing accounts for 74\% of Apple's total emissions while product use 19\%. In aggregate, the hardware life cycle (i.e., manufacturing, product transport, product use, recycling) accounts for over 98\% of the organization's total emissions.}
  \vspace{-1.0em}
  \label{fig:apple_breakdown}

\end{figure}

\section{Quantifying carbon emissions}~\label{sec:quantify_carbon}
Applications are run across a wide range of hardware platforms including wearables, mobile phones, personal assistants, and servers housed in datacenters.
For example, key-word spotting and speech recognition are run on personal assistants; web-browsing, media, image-classification and augmentation are run on mobile devices; large databases, scientific computing, and AI-based recommendation engines are run in the datacenter.
Recent work even explores partitioning workloads, including AI, AR/VR solutions, and data analysis across edge and datacenter hardware~\cite{autoscale, neurosurgeon, asplosARpaper}.
As tradeoffs between edge and datacenter execution evolve with emerging privacy aware systems and 5G communication technology, execution patterns for applications will continue to evolve as well.
Thus, anticipating emerging technology trends, it is important to quantify the carbon footprint over the wide range of hardware platforms.
Furthermore, estimates show that both consumer devices and datacenters are important to consider when optimizing environmental footprint as they account for 35\% and 25\% of global electricity demand, respectively.


%\textcolor{blue}{Brainstorm -- mapping AI training and inference computations to energy consumption, and from energy consumption to operational-related carbon emissions, and then extend to total (op plus cap) carbon emissions -- across different AI systems (with Fb's logged training runs, MLPerf's submission data?)}

To quantify the carbon footprint of hardware systems, we rely on two key methods: life cycle analyses (LCAs) and corporate reporting based on the Greenhouse Gas (GHG) protocol.


%One of the challenges in this domain is that it heavily depends on corporate disclosures of their operations.
%Typically this happens in one of two methods: life cycle analyses or following the GHG protocol.

% This is kind of like a methodology section

\subsection{Life cycle analyses}
Following Figure~\ref{fig:life_cycle}, LCAs quantify the carbon footprint from each individual process in the hardware life cycle. 
The process requires evaluating carbon emissions from procuring raw materials, transporting raw materials, producing tools and equipment to process the materials, designing and verifying systems, fabricating silicon wafers, assembling and packaging SoCs, shipping systems, using systems over their life time, and finally recycling hardware.
Carefully amortizing the emissions for each process for individual hardware units enables detailed carbon footprint analysis.
Unfortunately, accurate LCAs can be long and arduous to perform.

For the analysis shown in this paper, we build off of certified LCAs conducted by Apple, Microsoft, Google, Samsung, Huawei, and SK Hynix~\cite{}.
In particular, Apple, Microsoft, Samsung, Huawei, and Google publicly report LCAs for many mobile systems including phones (e.g., iPhones, Pixels, Matei), tablets (e.g., iPads, Surface, Galaxy), wearables (e.g., Apple Watch), and personal assistants (e.g., Google Home).
The life cycle analysis is typically assuming an average device lifetime of 3 years.
Finally, SK Hynix publicly reports LCAs for DRAM and NAND Flash memory systems~\cite{}.



\subsection{GHG protocol}
In addition to device level LCAs, organizations follow the Greenhouse Gas emissions~\cite{} protocol to report their carbon emissions. 
We use publicly available sustainability reports to analyze the GHG protocol-based emissions of datacenter oriented companies, such as Facebook and Google.

The GHG protocol categorizes emissions into three scopes which we define in the context of datacenter oriented companies below:
\begin{itemize}
\item \textbf{Scope 1:} Direct emissions from business activities. This includes emissions from diesel, natural gas, and refrigerants in offices and datacenters as well as, the diesel and gasoline for the transportation fleet owned and controlled by the company.
\item \textbf{Scope 2:} Indirect emissions in order to produce the electricity and heat. These emissions also include natural gas and purchased heat used to operate the offices and datacenters. Most importantly, scope 2 emissions include the footprint to generate the electricity driving all offices and datacenters.
\item \textbf{Scope 3:} Indirect emissions as a result of all other activities including the full supply chain. Scope 3 indirect emissions include the footprint to construct datacenters and manufacture server hardware.
\end{itemize}

Related to datacenter operations, Scope 2 comprises the operational or Opex-related carbon emissions while Scope 1 and Scope 3 comprise the capital or Capex-related carbon emissions.
While organizations following different accounting and disclosure practice, for the purposes of this study, we will use these reports to analyze overall datacenter carbon footprint trends.
We hope the initial characterization demonstrated here will motivate the need for detailed LCAs on datacenter scale hardware. 



==> text/pixel_hw_estimate.tex <==
\begin{table}[t!]
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Hardware} & \textbf{Estimate (g \co)} & \textbf{Actual (g \co)} & \textbf{Error (\%)} \\ \hline

Pixel 2 & 21.2 & 21.9 & -3.4 \\ \hline
Pixel 2 XL & 21.2 & 23.6 & -10.2 \\ \hline
Pixel 3 & 27.8 & 21.5 & +29.7 \\ \hline
Pixel 3 XL & 27.8 & 23.1 & +20.4 \\ \hline

\end{tabular}
\end{center}
\caption{ Estimating Pixel integrated circuit carbon footprint based on modeled SoC, memory, and storage overheads. 
Following Apple's breakdow, we assume \fixme{33}\% of carbon emissions for mobile devices come from integrated circuits.
The results show the first-order model to be within 9.2\% of reported emissions.}
\vspace{-1em}
\label{tab:pixel_hw_estimate}
\end{table}                                                                                                                                                                                                                                                                                                                 


==> text/relatedwork.tex <==
\section{Related work}

\textbf{Quantifying carbon footprint}

\textbf{Renewable energy aware scheduling}

\textbf{Datacenter scale optimization}

\textbf{Mobile optimization}



==> text/table_hw_CF.tex <==
\begin{table}[t!]
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Resource} & \textbf{Hardware} & \textbf{Carbon footprint} & \textbf{Unit} \\ \hline

DRAM & 50nm DDR3 & 600 & g CO2 per GB \\ \hline
DRAM & 40nm DDR3 & 315 & g CO2 per GB \\ \hline
DRAM & 30nm DDR3  & 230 & g CO2 per GB \\ \hline
DRAM & 30nm LPDDR3 & 201 & g CO2 per GB \\ \hline
DRAM & 20nm LPDDR3 & 184 & g CO2 per GB \\ \hline 
DRAM & 20nm LPDDR2 & 159 & g CO2 per GB \\ \hline \hline 
NAND & 30nm NAND & 31 & g CO2 per GB \\ \hline 
NAND & 20nm NAND & 15 & g CO2 per GB \\ \hline 
NAND & 10nm NAND & 10 & g CO2 per GB \\ \hline 
NAND & 1Z NAND TLC & 5.6 & g CO2 per GB \\ \hline  
NAND & V3 NAND TLC & 6.3 & g CO2 per GB \\ \hline  
NAND & Apple Disk & 8.6 $\pm$ 1.7 & g CO2 per GB \\ \hline  \hline
SOC & Mobile SoC & 273 $\pm$ 46 & g CO2 per mm$^2$ \\ \hline 
\end{tabular}
\end{center}
\caption{ Estimated carbon footprint of various memory, storage, and SoC hardware resources. 
DRAM and NAND Flash carbon footprints are based on SK Hynix's life cycle analysis.
SoC carbon footprints are estimated based on 33\% of Apple mobile phone's manufacturing footprint comes from integrated circuits --- SoC, DRAM, and NAND Flash}
\vspace{-1em}
\label{tab:hw_carbon}
\end{table}                                                                                                                                                                                                                                                                                                                 

